Horn Maximum Satisfiability: Reductions, Algorithms & Applications

Recent years have witness remarkable performance improvements in maximum satisfiability (MaxSAT) solvers. In practice, MaxSAT algorithms often target the most generic MaxSAT formulation, whereas dedicated solvers, which address specific subclasses of MaxSAT, have not been investigated. This paper shows that a wide range of optimization and decision problems are either naturally formulated as MaxSAT over Horn formulas, or permit simple encodings using Horn MaxSAT. Furthermore, the paper also shows how linear time decision procedures for Horn formulas can be used for developing novel algorithms for the Horn MaxSAT problem.

==> algs/maxhs.tex <==
%------------------------------------------------------------------------------%
% File:        maxhs.tex
%
% Description:
%
% Created:     13 Apr 2016.
%
% Author:      Joao Marques-Silva (jpms).
%------------------------------------------------------------------------------%
%
\input{algs/alg-defs}
%
\KwIn{$F$ WCNF formula}
\KwOut{$(\mu, \cost(\mu))$ MaxSAT assignment and cost}
%\KwOut{MCS $\fml{S}$}
%\BlankLine
\Begin{
  \SetAlgoVlined
  $K\gets \emptyset$ \;
  \While{\true}{
    $h \gets \minhs(K)$ \;
    $(\st,\mu)\gets\SAT(F\setminus h)$ \;
    \tcp{If $\st$, then $\mu $ is an assignment}
    \tcp{Otherwise, $\mu$ is a core}
    \lIf{$\st$}{\Return $(\mu, \cost(\mu))$}
    $K\gets K \cup \{\mu\}$\;
  }
}
\BlankLine
%
%------------------------------------------------------------------------------%


==> scratch.tex <==
%------------------------------------------------------------------------------%
% File:        scratch.tex
%
% Description: 
%
% Created:     13 Apr 2017.
%
% Author:      Joao Marques-Silva (jpms).
%------------------------------------------------------------------------------%

\section{Scratchpad}

\subsection{Introduction}

The maximum satisfiability (\mxsat) problem for Horn formulas
(\hmxsat) is well-known to be NP-hard~\cite{jaumard-ipl87}, whereas
the decision problem for Horn formulas is well-known to be solved in
linear time~\cite{gallier-jlp84,minoux-ipl88}.
%
Algorithms for the general \mxsat problem have seen remarkable
improvements in recent years~\cite{mhlpms-cj13}. These algorithms
propose different ways for iteratively finding and blocking
unsatisfiable cores (or subformulas).
%
One such family of algorithms~\cite{bacchus-cp11,jarvisalo-sat16},
which this paper refers to as \mxhs-like, consists of iteratively
computing a minimum hitting set $\fml{H}$ of a target formula
$\fml{T}$ (representing previously computed unsatisfiable cores) and
then checking the satisfiability of the original formula $\fml{F}$
without the computed minimum hitting $\fml{H}$.
%
If the original formula $\fml{F}$ is Horn, then each satisfiability
checking step can be done in \emph{linear time}.
%
This paper investigates a new family of \hmxsat algorithms building on
\mxhs-like~\cite{bacchus-cp11,jarvisalo-sat16} approaches.
%

This paper also shows that a wide range of optimization problems have
natural formulations as \hmxsat, including different optimization
problems over graphs or over sets. Furthermore, the paper remarks that
a large number of propositional encodings, some of which in practical
use for more than a decade, corresponds to Horn formulas. As a result,
a large number of practical applications where SAT and \mxsat have
found success can be shown to be solving \hmxsat optimization
problems.




%------------------------------------------------------------------------------%

